Perturbative theory of ensemble-averaged atomic dynamics in fluctuating laser fields

We have developed a perturbative method to model the resonant ionization of atomic systems in fluctuating laser fields. The perturbative method is based on an expansion in terms of the multitime cumulants, a suitable combination of moments (field's coherence functions), used to represent the field's statistical properties. The second-order truncated expansion is expressed in terms of the radiation's power spectrum and the intensity autocorrelation function. We investigate the range of validity of the model in terms of the field's coherence temporal length and peak intensity and have compared the results with conventional Monte-Carlo calculations. We apply the theory in the case of a near-resonant ionization of the Helium 2s2p autoionizing state with a SASE FEL pulse with square-exponentially dependent 1st-order coherence function. The ionization lineshape profile acquires a Voight profile; the degree of the Gaussian or Lorentzian character of which to depend crucially on the field's coherence time.

==> abstract.tex <==
% !TEX root = main.tex

We have developed a perturbative method to model the resonant ionization of atomic systems in fluctuating laser fields. The perturbative method is based on an expansion of the multitime cumulants of the stochastic field instead of its multitime moments (field's coherence functions). The second-order truncated expansion is expressed in terms of the radiation's power spectrum and the intensity autocorrelation function. We investigate the range of validity of the model in terms of the field's coherence temporal length and peak intensity and have compared the results with conventional Monte-Carlo calculations. We apply the theory in the case of a near-resonant ionization of the helium $2s2p$ autoionizing state with a SASE FEL pulse with square-exponentially dependent 1st-order coherence function. We show the ionization lineshape profile acquires a Voight profile; the Gaussian character of which to depend exclusively on the field's coherence function and its Lorentzian part to reflect the atomic structure of the system.         


%
%on the ionisation yields atom are modelled via Monte Carlo method and the approach of %averaging the time dependent density matrices (TDDM). The yield shapes obtained from %the two approaches are compared in different scenarios of the FEL using three sets of %key parameters. The averaging approach is computationally fast, whereas the Monte %Carlo method - even though it emulates an experimental scenario - is highly time %consuming. We show that averaging approach gives close results to that of the Monte %Carlo for low coherence times and low intensities. The correlation effects of the %field, determined by the shape of the autocorrelation function, have also been studied %using the averaging approach. A Gaussian correlated field (suits best for SASE-FELs) %give different yield shapes to that of a Lorentzian correlated field (generally suits %long-wavelength pulses). It is observed that the pulse duration plays a prominent role %in determining the difference between the effects of the two aforementioned %correlation types. Some approximations, which simplify the computations, without %jeopardising the accuracy of the results, have also been discussed.
%

==> diags/schematic2.tex <==



% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_b2pc1swz7 lines}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_b2pc1swz7}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfpointorigin}
\pgfpathlineto{\pgfpoint{\mcSize}{0}}
\pgfusepath{stroke}}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_r7s65ezz0 lines}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_r7s65ezz0}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfpointorigin}
\pgfpathlineto{\pgfpoint{\mcSize}{0}}
\pgfusepath{stroke}}}
\makeatother
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{figure}

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,471); %set diagram left start at 0, and has height of 471

%Straight Lines [id:da351717941082087] 
\draw [line width=2.25]    (178,374) -- (377.34,373.11) ;
%Straight Lines [id:da681678447785574] 
\draw [line width=2.25]    (170,230) -- (377.34,228.11) ;
%Shape: Rectangle [id:dp4860900293994419] 
\draw  [color={rgb, 255:red, 134; green, 40; blue, 40 }  ,draw opacity=1 ][pattern=_b2pc1swz7,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 122; green, 32; blue, 32}] (322,184.11) -- (504.34,184.11) -- (504.34,294) -- (322,294) -- cycle ;
%Straight Lines [id:da7630845829228772] 
\draw [color={rgb, 255:red, 126; green, 22; blue, 37 }  ,draw opacity=1 ][line width=2.25]    (281.19,372.63) -- (354.02,233.54) ;
\draw [shift={(356.34,229.11)}, rotate = 477.64] [fill={rgb, 255:red, 126; green, 22; blue, 37 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Shape: Wave [id:dp8261360608896438] 
\draw   (73.58,293.16) .. controls (72.88,296.2) and (72.21,299.09) .. (72.96,299.4) .. controls (73.71,299.72) and (75.68,297.37) .. (77.73,294.9) .. controls (79.79,292.42) and (81.76,290.07) .. (82.51,290.39) .. controls (83.26,290.7) and (82.59,293.59) .. (81.89,296.63) .. controls (81.18,299.66) and (80.51,302.56) .. (81.27,302.87) .. controls (82.02,303.18) and (83.98,300.83) .. (86.04,298.36) .. controls (88.1,295.89) and (90.06,293.54) .. (90.81,293.85) .. controls (91.57,294.17) and (90.9,297.06) .. (90.19,300.09) .. controls (89.49,303.13) and (88.82,306.02) .. (89.57,306.34) .. controls (90.32,306.65) and (92.29,304.3) .. (94.35,301.83) .. controls (96.41,299.36) and (98.37,297) .. (99.12,297.32) .. controls (99.87,297.63) and (99.2,300.52) .. (98.5,303.56) .. controls (97.79,306.6) and (97.13,309.49) .. (97.88,309.8) .. controls (98.63,310.12) and (100.59,307.76) .. (102.65,305.29) .. controls (104.71,302.82) and (106.67,300.47) .. (107.43,300.78) .. controls (108.18,301.1) and (107.51,303.99) .. (106.8,307.03) .. controls (106.1,310.06) and (105.43,312.95) .. (106.18,313.27) .. controls (106.94,313.58) and (108.9,311.23) .. (110.96,308.76) .. controls (113.02,306.29) and (114.98,303.94) .. (115.73,304.25) .. controls (116.48,304.56) and (115.82,307.46) .. (115.11,310.49) .. controls (114.41,313.53) and (113.74,316.42) .. (114.49,316.73) .. controls (115.24,317.05) and (117.2,314.7) .. (119.26,312.22) .. controls (121.32,309.75) and (123.29,307.4) .. (124.04,307.72) .. controls (124.79,308.03) and (124.12,310.92) .. (123.42,313.96) .. controls (122.71,316.99) and (122.04,319.89) .. (122.8,320.2) .. controls (123.55,320.51) and (125.51,318.16) .. (127.57,315.69) .. controls (129.63,313.22) and (131.59,310.87) .. (132.34,311.18) .. controls (133.1,311.5) and (132.43,314.39) .. (131.72,317.42) .. controls (131.02,320.46) and (130.35,323.35) .. (131.1,323.67) .. controls (131.85,323.98) and (133.82,321.63) .. (135.88,319.16) .. controls (137.93,316.69) and (139.9,314.33) .. (140.65,314.65) .. controls (141.4,314.96) and (140.73,317.85) .. (140.03,320.89) .. controls (139.32,323.93) and (138.66,326.82) .. (139.41,327.13) .. controls (139.65,327.23) and (140.01,327.06) .. (140.46,326.7) ;
%Straight Lines [id:da06620882351980417] 
\draw [color={rgb, 255:red, 121; green, 204; blue, 191 }  ,draw opacity=1 ][line width=1.5]    (62.95,288.38) -- (153.36,327.32) ;
\draw [shift={(156.11,328.5)}, rotate = 203.3] [color={rgb, 255:red, 121; green, 204; blue, 191 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Brace [id:dp8510518036670125] 
\draw  [color={rgb, 255:red, 21; green, 110; blue, 19 }  ,draw opacity=1 ] (204.19,254.63) .. controls (207.14,254.51) and (208.56,252.97) .. (208.45,250.02) -- (208.45,250.02) .. controls (208.28,245.8) and (209.67,243.63) .. (212.62,243.52) .. controls (209.67,243.63) and (208.11,241.58) .. (207.94,237.37)(208.02,239.26) -- (207.94,237.37) .. controls (207.83,234.42) and (206.29,233) .. (203.34,233.11) ;
%Straight Lines [id:da4490481842071863] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (193.19,260.63) -- (302.34,260.11) ;
%Curve Lines [id:da6634825223106675] 
\draw [color={rgb, 255:red, 152; green, 11; blue, 28 }  ,draw opacity=1 ][line width=2.25]  [dash pattern={on 6.75pt off 4.5pt}]  (233.34,230.11) .. controls (265.51,194.04) and (314.8,180.78) .. (353.39,225.55) ;
\draw [shift={(356.34,229.11)}, rotate = 231.48] [fill={rgb, 255:red, 152; green, 11; blue, 28 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Shape: Rectangle [id:dp8862680108931666] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][pattern=_r7s65ezz0,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 25; green, 40; blue, 155}] (304,21.11) -- (493,21.11) -- (493,126) -- (304,126) -- cycle ;
%Straight Lines [id:da6937455893099138] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (233.34,230.11) -- (349.55,57.26) ;
\draw [shift={(352.34,53.11)}, rotate = 483.91] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da24921872105435905] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (356.34,229.11) -- (446.64,88.32) ;
\draw [shift={(449.34,84.11)}, rotate = 482.68] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Curve Lines [id:da7459735197079675] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (258.77,262.37) .. controls (283.34,300.11) and (282.34,335.11) .. (263.34,371.11) ;
%Curve Lines [id:da7775671710085275] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (247.77,262.37) .. controls (232.34,297.11) and (227.34,338.11) .. (252.34,371.11) ;
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ] (235.94,268.26) -- (247.56,262.87) -- (251.34,275.11) ;
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ] (254.61,358.33) -- (253.08,371.84) -- (240.1,367.79) ;
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ] (273.22,367.26) -- (262.56,372.59) -- (259.34,361.11) ;
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ] (255.34,275.11) -- (259.23,263.13) -- (271.11,267.35) ;

% Text Node
\draw (119.92,320.74) node  [rotate=-13.65] [align=left] {};
% Text Node
\draw (155,374) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,xslant=-0.05] [align=left] {$\displaystyle |g\rangle $};
% Text Node
\draw (147,233) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,xslant=-0.05] [align=left] {$\displaystyle |a\rangle $};
% Text Node
\draw (522,248) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,xslant=-0.05] [align=left] {$\displaystyle |c\rangle $};
% Text Node
\draw (206,310) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,xslant=-0.05] [align=left] {$\displaystyle \textcolor[rgb]{0.25,0.46,0.02}{D\mathcal{E}( t)}$};
% Text Node
\draw (319,328) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,rotate=-297.13,xslant=-0.15] [align=left] {$\displaystyle \textcolor[rgb]{0.38,0.02,0.07}{\gamma _{g} \ ( t)}$};
% Text Node
\draw (300,181) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,xslant=-0.05] [align=left] {$\displaystyle \textcolor[rgb]{0.55,0.05,0.11}{\Gamma _{\alpha }}$};
% Text Node
\draw (114.87,290.7) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,rotate=-28.09,xslant=-0.05] [align=left] {$\displaystyle \omega _{r}$};
% Text Node
\draw (101.75,323.53) node  [rotate=-25.47] [align=left] {FEL};
% Text Node
\draw (511,75) node  [font=\large,color={rgb, 255:red, 27; green, 37; blue, 14 }  ,opacity=1 ,xslant=-0.05] [align=left] {$\displaystyle |c'\rangle $};
% Text Node
\draw (260,244) node   [align=left] {$\displaystyle E_{a} -E_{g} -\omega _{r}$};
% Text Node
\draw (256,124) node  [font=\large,color={rgb, 255:red, 7; green, 50; blue, 100 }  ,opacity=1 ,rotate=-304.77,xslant=-0.15] [align=left] {$\displaystyle \textcolor[rgb]{0.05,0.25,0.5}{\gamma _{a} \ ( t)}$};
% Text Node
\draw (391,144) node  [font=\large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-305.71,xslant=-0.15] [align=left] {$\displaystyle \textcolor[rgb]{0.04,0.21,0.42}{\gamma _{c} \ ( t)}$};


\end{tikzpicture}
\caption{Ionization scheme}
\end{figure}
